Towards Seamless Tracking-Free Web: Improved Detection of Trackers via One-class Learning

Numerous tools have been developed to aggressively block the execution of popular JavaScript programs (JS) in Web browsers. Such blocking also affects functionality of webpages and impairs user experience. As a consequence, many privacy preserving tools (PP-Tools) that have been developed to limit online tracking, often executed via JS, may suffer from poor performance and limited uptake. A mechanism that can isolate JS necessary for proper functioning of the website from tracking JS would thus be useful. Through the use of a manually labelled dataset composed of 2,612 JS, we show how current PP-Tools are ineffective in finding the right balance between blocking tracking JS and allowing functional JS. To the best of our knowledge, this is the first study to assess the performance of current web PP-Tools. To improve this balance, we examine the two classes of JS and hypothesize that tracking JS share structural similarities that can be used to differentiate them from functional JS. The rationale of our approach is that web developers often borrow and customize existing pieces of code in order to embed tracking (resp. functional) JS into their webpages. We then propose one-class machine learning classifiers using syntactic and semantic features extracted from JS. When trained only on samples of tracking JS, our classifiers achieve an accuracy of 99%, where the best of the PP-Tools achieved an accuracy of 78%. We further test our classifiers and several popular PP-Tools on a corpus of 4K websites with 135K JS. The output of our best classifier on this data is between 20 to 64% different from the PP-Tools. We manually analyse a sample of the JS for which our classifier is in disagreement with all other PP-Tools, and show that our approach is not only able to enhance user web experience by correctly classifying more functional JS, but also discovers previously unknown tracking services.

==> fselection.tex <==
%To the form the basis of statistical analysis of JavaScript code corpus, we develop and use method to extract meaningful code snippets ("semantic tokens") from the raw source code for all scrapped JavaScripts from the top 5,000 websites. The standard $n-gram$ statistical method used in NLP applications relies on certain property of natural language text: the context of a token is reasonably captured by the proceeding
%words, and the text tokens are different enough to have distinctive distributions, but common enough that a single text token be observed multiple times. Programming language does not obviously have these features: programs have complicated
%dependencies among non-sequential tokens, some programming language tokens are so common (e.g., $int$, $\{$, etc) that
%it is unclear what information they carry, and other tokens (e.g., variable or function names) are so idiosyncratic that it is unclear how to count them across multiple programs. Thus we augment our tracking classification scheme with the construction of useful "semantic tokens" from raw JavaScripts; these are small abstracted version of programming
%code under which the $n-gram$ counting model can be applied.
The key rationale behind our classification approach is the assumption that functional JavaScripts are similar to one another while being distinct from tracking JavaScripts and vice versa. Consider for instance the cookie setting code snippets from Google Analytics and Visual Revenue\footnote{Web analytics: \url{http://visualrevenue.com}} shown in Listings~\ref{lst:gacookiesetting} and \ref{lst:vrcookiesetting} respectively. These are examples of tracking JavaScripts. We can observe that the two are functionally and structurally similar, with differences in variable names. Likewise, the tracking code snippets from Google Analytics and Effective Measurements\footnote{Web analytics: \url{http://effectivemeasure.com}} in Listings~\ref{lst:gatracking} and \ref{lst:emtracking} are similar. 
\lstdefinelanguage{MyScript}{
}
\lstset{
	tabsize=2,
	basicstyle=\footnotesize\ttfamily,
	showstringspaces=false,
	showspaces=false,
	language=MyScript
}
\begin{lstlisting}[caption={Google Analytics Cookie Setting},frame=single, label={lst:gacookiesetting},escapeinside={@}{@}]
var _gaq = _gaq || [];
_gaq.push(['_setAccount', 'UA-1627489-1']);
_gaq.push(['_setDomainName', 'geo.tv']);
_gaq.push(['_trackPageview']);
\end{lstlisting}
\begin{lstlisting}[caption={Visual Revenue Cookie Setting},frame=single, label={lst:vrcookiesetting},escapeinside={@}{@}]
var _vrq = _vrq || [],
_vrqIsOnHP = (document.body.className || 
	'').search('pg-section')&gt;=0 
	? true : false;
_vrq.push(['id', 396]);
_vrq.push(['automate', _vrqIsOnHP]);
_vrq.push(['track', function() {}]);
\end{lstlisting}
\begin{lstlisting}[caption={Google Analytics Tracking Script},frame=single, label={lst:gatracking},escapeinside={@}{@}]
 (function() {
   var ga=document.createElement('script');
   ga.type = 'text/javascript';
   ga.async = true;
   ga.src = ('https:' == document.
   location.protocol ? 'https:
   //ssl' : 'http://www') 
   + '.google-analytics.com/ga.js';
   var s = document.getElementsByTagName
   ('script')[0];
   s.parentNode.insertBefore(ga, s);
 })();
\end{lstlisting}

\begin{lstlisting}[caption={Effective Measurement Tracking Script},frame=single, label={lst:emtracking},escapeinside={@}{@}]
(function() {
  var em=document.createElement('script');
  em.type = 'text/javascript';
  em.async = true;
  em.src = ('https:' == document.
  location.protocol ? 'https://
  pk-ssl' : 'http://pk-cdn') + 
  '.effectivemeasure.net/em.js';
  var s = document.getElementsByTagName
  ('script')[0];
  s.parentNode.insertBefore(em, s);
})();
\end{lstlisting}

These examples indicate that a similarity measure based on a feature space composed of semantic or syntactic tokens from these JavaScripts should be effective in differentiating between functional and tracking JavaScripts. Before we give details of the syntactic and semantic models, we define a few terms. Let $H$ denote the set of (HTML) web-pages belonging to the given dataset (in our case, $H$ could be the labelled or the wild dataset). Let $J$ denote the set of all JavaScripts present in the web-pages from $H$. Given an $h \in H$, the function $\mathsf{js}$ returns the set of JavaScripts contained in $h$, such that the following holds
\[
\bigcup_{h \in H} \mathsf{js}(h) = J.
\]
Let $P$ denote a PP-Tool. Then $P(h)$ denotes the DOM tree obtained after applying $P$ to $h$. We also introduce the identity PP-Tool denoted $I$, such that $I(h) = h$. We have the condition
\[
\mathsf{js}(P(h)) \subseteq \mathsf{js}(h),
\]
from which it follows that the ratio
\[
a_{P}(h) = 1 - \frac{\lvert \mathsf{js}(P(h)) \rvert}{ \lvert \mathsf{js}(h) \rvert},
\]
is within the interval $[0, 1]$. We call this the \emph{aggression coefficient}. Note that $a_{I}(h) = 0$ for all $h \in H$. This is called the baseline. A PP-Tool $P$ is said to be \emph{aggressive on $h$} if it has a high aggression coefficient when applied to $h$. This means that the PPTool removes most of the JavaScripts from the webpage in question. A PP-Tool is said to be \emph{aggressive} if it has a high aggression coefficient for a high portion of web-pages from $H$. Where we talk of a generic $h$, we may simply use $a_P$ instead of $a_{P}(h)$. 

To quantitatively measure similarity between different JavaScripts, we use the \textit{term frequency with inverse document frequency} measure, denoted $\mathsf{tf}\text{-}\mathsf{idf}$. Central to this measure is the term $t$. How the term $t$ is defined gives rise to the different semantic and syntactic models to be discussed shortly. For now let us assume that each JavaScript $j \in J$ is composed of one or more terms. We then use the boolean term frequency ($\mathsf{tf}$) measure such that $\mathsf{tf}(t, j) = 1$ if $t \in j$ and $0$ otherwise. The inverse document frequency 
measure \textsf{idf} is defined as:
\[
\mathsf{idf}(t, j, J) = \log \frac{|J|}{\lvert \{j \in J : t \in j \} \rvert}
\]
Finally, we obtain $\mathsf{tf}$ with $\mathsf{idf}$ for each $t \in j$ over the corpus $J$, as:
% As future work, we anticipate to use n-gram measures over program dependency graph 
% to capture JavaScript structure and semantics. 
%  We deem that this will improve our overall results of our systems. 
\begin{equation*}
\mathsf{tf} \text{-} \mathsf{idf}(t, j, J) = \mathsf{tf}(t, j)\cdot \mathsf{idf}(t, j, J).
\label{eq:2}
\end{equation*}
Note that, intuitively, the \textsf{tf}\text{-}\textsf{idf} measure gives more weight to terms that are less common in $J$, since such terms are more likely to make the corresponding JavaScript stand out. The \textsf{tf}\text{-}\textsf{idf} thus transforms our corpus $J$ to the feature vector space. The feature vector corresponding to JavaScipt $j$ is denoted by $\mathbf{j}$. The $i$th component of $\mathbf{j}$, denoted $\mathbf{j}[i]$ corresponds to the term $t_i$ and is equal to $\mathsf{tf} \text{-} \mathsf{idf}(t_i, j, J)$. It is assumed that all possible terms occurring in $J$ are enumerated.

\subsection{Syntactic Model}
In the syntactic model, the term $t$ is defined as a string of characters representing \textit{one line} of JavaScript code.  Due to a large number of JavaScripts contained in $J$ the dimension of the resulting feature space can become very large. We therefore ``cap'' the feature vector space by only considering the top \textcolor{red}{200} terms as ranked by their \textsf{tf}\text{-}\textsf{idf} scores. 

\subsection{Semantic Models}
\label{subsec:ngramdm}
The above mentioned syntactic model is good as a base point. We are however, also interested in a richer model that captures 
the structure of JavaScripts. For this we resort to the $n$-gram model introduced in \cite{Hsiao:2014:oopsala}. The approach identifies 
tokens in programs whose importance can then be determined through some statistical measure such as \textsf{tf}-\textsf{idf}. An example 
of a token is one line of JavaScript code, as used in the syntactic model. An $n$-gram where $n \ge 1$ refers to multiple tokens which are 
in some sense dependent on each other. To construct $n$-grams, the approach taken in \cite{Hsiao:2014:oopsala} converts the code into 
a \emph{canonical form}. From this canonical form, two different models can be derived based on how the $n$-grams are constructed. The difference lies in how different lines 
of the canonical code are perceived to be dependent on each other. One way is sequential dependency, where a line of code is dependent on the execution of the 
previous line, and so on. We call this the sequential $n$-gram model. 

Since consecutive lines in source code are often unrelated to each other, instead of computing $n$-grams via this 
trivial ordering, program dependency graphs (PDGs) can be employed  \cite{Muchnick:1998:ACD, Hsiao:2014:oopsala}. In such a graph, a node 
represents a single statement from the canonical form. A node $a$ of the graph is dependent on a node $b$ if its execution depends on the 
result of $b$ or if it takes as input a value written by $b$. If this is true node $a$ is connected to $b$ via a directed edge in the direction of the latter. 
An $n$-gram of a particular gram $x$ is then the subgraph of the program dependency graph consisting of all (backward) paths of length $n-1$ 
starting from $x$. See Appendix~\ref{sec:appendixA} for more details. We call this the PDG $n$-gram model.

Once $n$-grams have been constructed via the sequential or PDG model, we can use them in our \textsf{tf}-\textsf{idf} measure to calculate their relative importance as is done in \cite{Hsiao:2014:oopsala}. Thus, the term $t$ used in the \textsf{tf}-\textsf{idf} score for the two aforementioned semantic models is an $n$-gram. Finally, we can also have different models depending on the value of $n$ in $n$-gram. For our study, we use $4$-gram and $7$-gram variants. 



==> simpaper.bib-bak.tex <==
@inproceedings{TranDLJ12,
  author    = {Minh Tran and
               Xinshu Dong and
               Zhenkai Liang and
               Xuxian Jiang},
  title     = {Tracking the Trackers: Fast and Scalable Dynamic Analysis of Web Content
               for Privacy Violations},
  booktitle = {{ACNS}, 2012.}
 }
 
 @inproceedings{Basu:2004,
 author = {Basu, Sugato and Bilenko, Mikhail and Mooney, Raymond J.},
 title = {A Probabilistic Framework for Semi-supervised Clustering},
 booktitle = {{KDD}}, 
 year = {2004}
 }
 
 
 @article{Erman:2007,
 author = {Erman, Jeffrey and Mahanti, Anirban and Arlitt, Martin and Cohen, Ira and Williamson, Carey},
 title = {Offline/Realtime Traffic Classification Using Semi-supervised Learning},
 journal = {Perform. Eval.},
 year = {2007}
 }
 
@inproceedings{mayer2012third,
  title={Third-Party Web Tracking: Policy and Technology},
  author={Mayer, Jonathan R. and Mitchell, John C.},
  booktitle={{IEEE S\&P}, 2012}
}
@inproceedings{Jang:2010:ESP:,
 author = {Jang, Dongseok and Jhala, Ranjit and Lerner, Sorin and Shacham, Hovav},
 title = {An Empirical Study of Privacy-violating Information Flows in JavaScript Web Applications},
 booktitle = {{CCS}, 2010},
}
@inproceedings{Yue:2009:,
 author = {Yue, Chuan and Wang, Haining},
 title = {Characterizing Insecure Javascript Practices on the Web},
 series = {{WWW} 2009}
}
@inproceedings{Xu:2012:POT,
 author = {Xu, Wei and Zhang, Fangfang and Zhu, Sencun},
 title = {The Power of Obfuscation Techniques in Malicious JavaScript Code: A Measurement Study},
 series = {{MALWARE}, 2012}
} 
@inproceedings{Curtsinger:2011,
 author = {Curtsinger, Charlie and Livshits, Benjamin and Zorn, Benjamin and Seifert, Christian},
 title = {ZOZZLE: Fast and Precise In-browser JavaScript Malware Detection},
 booktitle = {Proceedings of the 20th USENIX Conference on Security},
 series = {{SEC}, 2011}
}

@inproceedings{Tran:2012:TTF:,
 author = {Tran, Minh and Dong, Xinshu and Liang, Zhenkai and Jiang, Xuxian},
 title = {Tracking the Trackers: Fast and Scalable Dynamic Analysis of Web Content for Privacy Violations},
 series = {{ACNS}, 2012}
} 

@inproceedings{conf/ndss/YenXYYA12,
  author = {Yen, Ting-Fang and Xie, Yinglian and Yu, Fang and Yu, Roger Peng and Abadi, Mart},
  booktitle = {NDSS, 2012},
  title = {Host Fingerprinting and Tracking on the Web: Privacy and Security Implications.}
}
@inproceedings{olejnik:hal-00747841,
  TITLE = {{Why Johnny Can't Browse in Peace: On the Uniqueness of Web Browsing History Patterns}},
  AUTHOR = {Olejnik, Lukasz and Castelluccia, Claude and Janc, Artur},
  BOOKTITLE = {{HotPETs}, 2012},
}
@inproceedings{Acar:2014:WNF:,
 author = {Acar, Gunes and Eubank, Christian and Englehardt, Steven and Juarez, Marc and Narayanan, Arvind and Diaz, Claudia},
 title = {The Web Never Forgets: Persistent Tracking Mechanisms in the Wild},
 booktitle = {{CCS}, 2014.}
}
@inproceedings{YuPEBL:2002,
 author = {Yu, Hwanjo and Han, Jiawei and Chang, Kevin Chen-Chuan},
 title = {PEBL: Positive Example Based Learning for Web Page Classification Using SVM},
 booktitle = {{KDD, 2002}}
} 
@inproceedings{Krishnamurthy:2009,
 author = {Krishnamurthy, Balachander and Wills, Craig},
 title = {Privacy Diffusion on the Web: A Longitudinal Perspective},
 booktitle = {{WWW} 2009}}
} 

@inproceedings{Mao:2011,
 author = {Mao, Huina and Shuai, Xin and Kapadia, Apu},
 title = {Loose Tweets: An Analysis of Privacy Leaks on Twitter},
 booktitle = {{WPES} 2011}}
 } 

@book{opac-b1130221,
   title = {Googling security : how much does Google know about you? Greg Conti},
   author = {Conti, Greg},
   publisher = {Addison-Wesley, 2009}
 }

@inproceedings{cujo,
 author = {Rieck, Konrad and Krueger, Tammo and Dewald, Andreas},
 title = {Cujo: Efficient Detection and Prevention of Drive-by-download Attacks},
 booktitle = {{ACSAC}, 2010}}
} 

@article{Muller:2001,
 author = {Muller, K. -R. and Mika, S. and Ratsch, G. and Tsuda, K. and Scholkopf, B.},
 title = {An Introduction to Kernel-based Learning Algorithms},
 journal = {{ToNN}, 2001}
} 
@article{Mayerthird-partyweb,
    author = {Jonathan R. Mayer and John C. Mitchell},
    title = {Third-party web tracking: Policy and technology},
    booktitle = {{S\&P}, 2012}
}
@inproceedings{Gill:2013,
 author = {Gill, Phillipa and Erramilli, Vijay and Chaintreau, Augustin and Krishnamurthy, Balachander and Papagiannaki, Konstantina and Rodriguez, Pablo},
 title = {Follow the Money: Understanding Economics of Online Aggregation and Advertising},
 booktitle = {{IMC}, 2013}
} 
@inproceedings{Ma:2009:,
 author = {Ma, Justin and Saul, Lawrence K. and Savage, Stefan and Voelker, Geoffrey M.},
 title = {Beyond Blacklists: Learning to Detect Malicious Web Sites from Suspicious URLs},
 booktitle = {{KDD}, 2009}
} 
@misc{easylist,
  title = {EasyList},
  howpublished = {\url{https://easylist-downloads.adblockplus.org/easylist.txt}},
  mynote = {{Accessed On}: 2015-05-01}
}

@misc{ganalytics,
  title = {Visual Revenue},
  howpublished = {\url{https://www.google.com/analytics/}},
  mynote = {{Accessed On}: 2015-05-01}
}
@misc{vrenue,
  title = {Visual Revenue},
  howpublished = {\url{http://www.visualrevenue.com}},
  mynote = {{Accessed On}: 2015-05-01}
}
@misc{moat,
  title = {Moat},
  howpublished = {\url{http://www.moat.com/}},
  mynote = {{Accessed On}: 2015-05-01}
}
@misc{disqus,
  title = {Disqus},
  howpublished = {\url{http://www.disqus.com/}},
  mynote = {{Accessed On}: 2015-05-01}
}

@misc{effpolicy,
  title = {{EFF DNT Policy}},
  howpublished = {\url{https://www.eff.org/dnt-policy}},
  mynote = {{Accessed On}: 2015-05-01}
}
@misc{seleniumhq,
  title = {{Selenium Webdriver}},
  howpublished = {\url{http://www.seleniumhq.org/}},
  mynote = {{Accessed On}: 2015-05-01}
}
@misc{pbdgerblocklist,
  title = {{Privacy Badger Cookies Blocklist}},
  howpublished = {\url{
https://github.com/EFForg/privacybadgerfirefox/blob/master/data/cookieblocklist.txt
}},
  mynote = {{Accessed On}: 2015-05-01}
}
@misc{Pagefair,
  title = {{PageFair: Why aren't PageFair Ads blocked?}},
  howpublished = {\url{https://pagefair.com/about/}},
  mynote = {{Accessed On}: 2015-08-14}
}

@misc{ghostery,
  title = {{Ghostery}},
  howpublished = {\url{https://www.ghostery.com}},
  mynote = {{Accessed On}: 2015-05-04}
}
@misc{adblockplus,
  title = {{Adblock Plus}},
  howpublished = {\url{https://www.adblockplus.org}},
  mynote = {{Accessed On}: 2015-07-02}
}
@misc{noscript,
  title = {{NoScript}},
  howpublished = {\url{https://www.noscript.net}},
  mynote = {{Accessed On}: 2015-07-03}
}
@misc{ssscript,
  title = {{Surrogate JavaScript Code}},
  howpublished = {\url{https://news.ycombinator.com/item?id=5182359}},
  mynote = {{Accessed On}: 2015-07-04}
}

@misc{ssscript1,
  title = {{NoScript's Surrogates JavaScript Code}},
  howpublished = {\url{https://hackademix.net/2011/09/29/script-surrogates-quick-reference/}},
  mynote = {{Accessed On}: 2015-07-04}
}

@misc{privacybadger,
  title = {{Privacy Badger}},
  howpublished = {\url{https://www.eff.org/privacybadger}},
  mynote = {{Accessed On}: 2015-07-07}
}

@misc{disconnect,
  title = {{Disconnect}},
  howpublished = {\url{https://www.disconnect.me/}},
  mynote = {{Accessed On}: 2015-07-04}
}
@misc{fanboylist,
  title = {FanboyList},
  howpublished = {\url{https://easylist-downloads.adblockplus.org/fanboy-social.txt}},
  mynote = {{Accessed On}: 2015-07-01}
}
. .
@misc{Tor,
  title = {Tor Project: Anonymity Online},
  howpublished = {\url{https://www.torproject.org/}},
  mynote = {{Accessed On}: 2015-07-01}
}
@article{ref1,
  author={David Gugelmann, Bernhard Ager, Vincent Lenders},
  title={An Automated Approach for complementing Ad blcokers' blacklists},
  booktitle={{PETS}, 2015}
}
@inproceedings{ikram:2014,
  title={On the Intrusiveness of JavaScript on the Web},
  author={Ikram, Muhammad and Asghar, Hassan and Kaafar, Mohamed Ali and Mahanti, Anirban},
  booktitle={{CoNEXT}, 2014}
}
@inproceedings{Orr:2012,
	title = {An Approach for Identifying JavaScript-loaded Advertisements Through Static Program Analysis},
	Author = {Orr, Caitlin R. and Chauhan, Arun and Gupta, Minaxi and Frisz, Christopher J. and Dunn, Christopher W.},
	Booktitle = {{WPES}, 2012}
}

@inproceedings{ref11,
 author = {Gugelmann, David and Ager, Bernhard and Lenders, Vincent},
  title={An Automated Approach for complementing Ad blcokers' blacklists},
  booktitle={{PETs}, 2015}
}

@INPROCEEDINGS{4740447, 
author={Papadopoulou, E. and McBurney, S. and Taylor, N. and Williams, M.H.}, 
booktitle={{WIIAT}, 2008}, 
title={Linking Privacy and User Preferences in the Identity Management for a Pervasive System}, 
year={2008} 
}
@inproceedings{Dong:2011,
 author = {Dong, Xinshu and Tran, Minh and Liang, Zhenkai and Jiang, Xuxian},
 title = {AdSentry: Comprehensive and Flexible Confinement of JavaScript-based Advertisements},
 booktitle = {{ACSAC}, 2011}}
} 

@misc{brokenpages,
  title = {{Ghostery} Blocking Breaks WebPage Functionalities},
  howpublished = {\url{http://tinyurl.com/ov6f9j9}},
  mynote = {{Accessed On}: 2015-07-01}
}

@misc{trackingtrackers,
  title = {Tracking the Trackers},
  howpublished = {\url{http://cyberlaw.stanford.edu/node/6730}},
  mynote = {[{Accessed On}: 2015-05-01]}
}
@article{Lederer:2004:PPT,
 author = {Lederer, Scott and Hong, Jason I. and Dey, Anind K. and Landay, James A.},
 title = {Personal Privacy Through Understanding and Action: Five Pitfalls for Designers},
 journal = {Personal Ubiquitous Comput., 2004}
} 

@inproceedings{Ha:2006:EUP,
 author = {Ha, Vicki and Inkpen, Kori and Al Shaar, Farah and Hdeib, Lina},
 title = {An Examination of User Perception and Misconception of Internet Cookies},
 booktitle = {{CHI}, 2006}
} 

@article{Cranor:2006:UIP,
 author = {Cranor, Lorrie Faith and Guduru, Praveen and Arjula, Manjula},
 title = {User Interfaces for Privacy Agents},
 journal = {ACM {ToCHI}, 2006}
} 
@article{Krishnamurthy:2010,
 author = {Krishnamurthy, Balachander},
 title = {I Know What You Will Do Next Summer},
 journal = {SIGCOMM {CCR}, 2010}
} 

@inproceedings{Krishnamurthy:2007,
 author = {Krishnamurthy, Balachander and Malandrino, Delfina and Wills, Craig E.},
 title = {Measuring Privacy Loss and the Impact of Privacy Protection in Web Browsing},
 booktitle = {{SOUPS}, 2007}
}
@inproceedings{Balaprivacyleakage:2011,
author = {Balachander Krishnamurthy and Konstantin Naryshkin and Craig Wills},
title = {Privacy leakage vs. Protection measures: the growing disconnect},
booktitle = {{W2SP}, 2011}
}
@article{YuSingleClass:2005,
 author = {Yu, Hwanjo},
 title = {Single-Class Classification with Mapping Convergence},
 journal = {{ML}, 2005}
} 

@article{WangPSOL:2006,
 author = {Wang, Chunlin and Ding, Chris and Meraz, Richard F. and Holbrook, Stephen R.},
 title = {PSoL: A Positive Sample Only Learning Algorithm for Finding Non-coding RNA Genes},
 journal = {Bioinformatics, 2006}
}

@article{FungTextClassification:2006,
 author = {Fung, Gabriel Pui Cheong and Yu, Jeffrey X. and Lu, Hongjun and Yu, Philip S.},
 title = {Text Classification Without Negative Examples Revisit},
 journal = {IEEE {ToKDE}, 2006}
} 

@INPROCEEDINGS{Lee03learningwith,
    author = {Wee Sun Lee and Bing Liu},
    title = {Learning with Positive and Unlabeled Examples Using Weighted Logistic Regression},
    booktitle = {{ICML}, 2003}
}
@inproceedings{LiuPositiveLables:2003,
 author = {Liu, Bing and Dai, Yang and Li, Xiaoli and Lee, Wee Sun and Yu, Philip S.},
 title = {Building Text Classifiers Using Positive and Unlabeled Examples},
 booktitle = {{ICDM}, 2003}
} 
@inproceedings{Elkan:2008,
 author = {Elkan, Charles and Noto, Keith},
 title = {Learning Classifiers from Only Positive and Unlabeled Data},
 booktitle = {{KDD}, 2008}
} 
@ARTICLE{oneclass, 
author={Wenkai Li and Qinghua Guo and Elkan, C.}, 
journal={{ToGRS}, 2011}, 
title={A Positive and Unlabeled Learning Algorithm for One-Class Classification of Remote-Sensing Data}
}
@article{Manevitz:2002:OSD,
 author = {Manevitz, Larry M. and Yousef, Malik},
 title = {One-class Svms for Document Classification},
 journal = {{MLR}, 2002}
} 
@article{Chang:2011:LibSVM,
 author = {Chang, Chih-Chung and Lin, Chih-Jen},
 title = {LIBSVM: A Library for Support Vector Machines},
 journal = {ACM {ToIST}, 2011}
} 

@article{scikit-learn,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa F et al.,},
 journal={{MLR}, 2011}
}
@MISC{Denis02textclassification,
    author = {François Denis and R\'emi Gilleron and Marc Tommasi},
    title = {Text Classification from Positive and Unlabeled Examples},
    year = {2002}
}
@INPROCEEDINGS{Denis98paclearning,
    author = {Francois Denis},
    title = {PAC Learning from Positive Statistical Queries},
    booktitle = {{ALT}, 1998}
}
@INPROCEEDINGS{Zhang05asimple,
    author = {Dell Zhang},
    title = {A Simple Probabilistic Approach to Learning from Positive and Unlabeled Examples},
    booktitle = {{WCI}, 2005}
}
@article{Scholkopf:2001:ESH,
 author = {Sch\"{o}lkopf, Bernhard and Platt, John C. and Shawe-Taylor, John C. and Smola, Alex J. and Williamson, Robert C.},
 title = {Estimating the Support of a High-Dimensional Distribution},
 journal = {{NC}, 2001}
} 

@article{Tax:2004:SVD,
 author = {Tax, David M. J. and Duin, Robert P. W.},
 title = {Support Vector Data Description},
 journal = {{ML}, 2004}
} 

@book{Aho:CT:2006,
 author = {Aho, Alfred V. and Lam, Monica S. and Sethi, Ravi and Ullman, Jeffrey D.},
 title = {Compilers: Principles, Techniques, and Tools (2Nd Edition)},
 publisher = {Addison-Wesley Longman Publishing Co., Inc., 2006}
} 
@INPROCEEDINGS{Brants07llmodel,
    author = {Thorsten Brants and Ashok C. Popat and Peng Xu and Franz J. Och and Jeffrey Dean and Google Inc},
    title = {Large language models in machine translation},
    booktitle = {{EMNLP}, 2007}
}
@incollection{SparckJones:1988,
 author = {Sparck Jones, Karen},
 chapter = {A Statistical Interpretation of Term Specificity and Its Application in Retrieval},
 title = {Document Retrieval Systems},
 editor = {Willett, Peter, 1998},
}
@inproceedings{Liblit:2005:SSB,
 author = {Liblit, Ben and Naik, Mayur and Zheng, Alice X. and Aiken, Alex and Jordan, Michael I.},
 title = {Scalable Statistical Bug Isolation},
 booktitle = {{PLDI}, 2005},
}

@inproceedings{Gabel:2008:SDS,
 author = {Gabel, Mark and Jiang, Lingxiao and Su, Zhendong},
 title = {Scalable Detection of Semantic Clones},
 booktitle = {{ICSE}, 2008}
} 

@inproceedings{Jiang:2007:DSA,
 author = {Jiang, Lingxiao and Misherghi, Ghassan and Su, Zhendong and Glondu, Stephane},
 title = {DECKARD: Scalable and Accurate Tree-Based Detection of Code Clones},
 booktitle = {{ICSE}, 2007}
} 

@inproceedings{Juergens:2009:CCM,
 author = {Juergens, Elmar and Deissenboeck, Florian and Hummel, Benjamin and Wagner, Stefan},
 title = {Do Code Clones Matter?},
 booktitle = {{ICSE}, 2009}
} 

@inproceedings{Khoo:2013:RSE,
 author = {Khoo, Wei Ming and Mycroft, Alan and Anderson, Ross},
 title = {Rendezvous: A Search Engine for Binary Code},
 booktitle = {{MSR}, 2013}
} 
@article{Li:2006:CFC,
 author = {Li, Zhenmin and Lu, Shan and Myagmar, Suvda and Zhou, Yuanyuan},
 title = {CP-Miner: Finding Copy-Paste and Related Bugs in Large-Scale Software Code},
 journal = {IEEE {ToSE}, 2006}
} 
@inproceedings{Nikiforakis:2012:,
 author = {Nikiforakis, Nick and Invernizzi, Luca and Kapravelos, Alexandros and Van Acker, Steven and Joosen, Wouter and Kruegel, Christopher and Piessens, Frank and Vigna, Giovanni},
 title = {You Are What You Include: Large-scale Evaluation of Remote Javascript Inclusions},
 booktitle = {{CCS}, 2012}
} 

@inproceedings{Nikiforakis:2013:CME,
 author = {Nikiforakis, Nick and Kapravelos, Alexandros and Joosen, Wouter and Kruegel, Christopher and Piessens, Frank and Vigna, Giovanni},
 title = {Cookieless Monster: Exploring the Ecosystem of Web-Based Device Fingerprinting},
 booktitle = {{IEEE S\&P}, 2013}}
} 
@inproceedings{Schleimer:2003:WLA, 
 author = {Schleimer, Saul and Wilkerson, Daniel S. and Aiken, Alex},
 title = {Winnowing: Local Algorithms for Document Fingerprinting},
 booktitle = {{SIGMOD} 2003}
} 
@inproceedings{Jang:2010:,
 author = {Jang, Dongseok and Jhala, Ranjit and Lerner, Sorin and Shacham, Hovav},
 title = {An Empirical Study of Privacy-violating Information Flows in JavaScript Web Applications},
 booktitle = {{CCS}, 2010}
} 
@inproceedings{Cai:2011:ESL,
 author = {Cai, Dongxiang and Kim, Miryung},
 title = {An Empirical Study of Long-lived Code Clones},
 booktitle = {{ETAPS}, 2011}
}

@INPROCEEDINGS{Gre12,
AUTHOR = {Pam Green and Peter C. R. Lane and Austen Rainer and Sven-Bodo Scholz and Steve Bennett},
TITLE = {Same Difference: Detecting Collusion by Finding Unusual Shared Elements},
BOOKTITLE = {{IPC}, 2012}
}
@INPROCEEDINGS{pptoolusage,
AUTHOR = {Hassan Metwalley, Stefano Traverso, Marco Mellia},
TITLE = {The Online Tracking Horde: a View from Passive Measurements},
BOOKTITLE = {{TMA}, 2015}
}

@inproceedings{Lucia:2011:IUC,
 author = {Lucia, Brandon and Wood, Benjamin P. and Ceze, Luis},
 title = {Isolating and Understanding Concurrency Errors Using Reconstructed Execution Fragments},
 booktitle = {{PLDI}, 2011}
} 

@inproceedings{Evans:2007:CDV,
 author = {Evans, William S. and Fraser, Christopher W. and Ma, Fei},
 title = {Clone Detection via Structural Abstraction},
 booktitle = {{WCRE}, 2007}
} 

@inproceedings{Hsiao:2014:oopsala,
 author = {Chun-Hung Hsiao and Michael Cafarella and Satish Narayanasamy},
 title = {Using Web Corpus Statistics for Program Analysis},
 booktitle = {{OOPSLA}, 2014}
} 
@article{Ferrante:1987:PDG,
 author = {Ferrante, Jeanne and Ottenstein, Karl J. and Warren, Joe D.},
 title = {The Program Dependence Graph and Its Use in Optimization},
 journal = {ACM {ToPLS}, 1987}
} 

@book{Muchnick:1998:ACD,
 author = {Muchnick, Steven S.},
 title = {Advanced Compiler Design and Implementation},
 publisher = {MK Publishers Inc., 1997}
} 

@inproceedings{roesner,
 author = {Roesner, Franziska and Kohno, Tadayoshi and Wetherall, David},
 title = {{Detecting and Defending Against Third-party Tracking on the Web}},
 booktitle = {{NSDI}, 2012}
} 

@inproceedings{WOSN2012,
 author = {Chaabane, Abdelberi and Kaafar, Mohamed Ali and Boreli, Roksana},
 title = {{Big Friend is Watching You: Analyzing Online Social Networks Tracking Capabilities}},
 booktitle = {{WOSN}, 2012}
} 

